Sirius: Contextual Sparsity with Correction for Efficient LLMs

With the blossom of large language models (LLMs), inference efficiency becomes increasingly important. Various approximation methods are proposed to reduce the cost at inference time. Contextual Sparsity (CS) is appealing for its training-free nature and its ability to reach a higher compression ratio seemingly without quality degradation. However, after a comprehensive evaluation of contextual sparsity methods on various complex generation tasks, we find that although CS succeeds in prompt-understanding tasks, CS significantly degrades the model performance for reasoning, deduction, and knowledge-based tasks. Despite the gap in end-to-end accuracy, we observed that sparse models often share general problem-solving logic and require only a few token corrections to recover the original model performance. This paper introduces Sirius, an efficient correction mechanism, which significantly recovers CS models quality on reasoning tasks while maintaining its efficiency gain. Sirius is evaluated on 6 models with 8 difficult generation tasks in reasoning, math, and coding and shows consistent effectiveness and efficiency. Also, we carefully develop a system implementation for Sirius and show that Sirius achieves roughly 20% reduction in latency for 8B model on-chip and 35% reduction for 70B model offloading. We open-source our implementation of Sirius at https://github.com/Infini-AI-Lab/Sirius.git.

==> Styles/oldexperimentnotes.tex <==
% only correcting tokens but not roll back: Not helping
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=True,kernel_size=16,spr=0.5,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.5815|±  |0.0136|
% |     |       |flexible-extract|     5|exact_match|0.5876|±  |0.0136|
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=True,kernel_size=16,spr=0.5,thr=0.2), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.5754|±  |0.0136|
% |     |       |flexible-extract|     5|exact_match|0.5807|±  |0.0136|
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=True,kernel_size=16,spr=0.5,thr=0.3), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.5679|±  |0.0136|
% |     |       |flexible-extract|     5|exact_match|0.5732|±  |0.0136|



correct 

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=False,kernel_size=16,spr=0.5,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value|   |Stderr|
% |-----|------:|----------------|-----:|-----------|----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.580|±  |0.0136|
% |     |       |flexible-extract|     5|exact_match|0.583|±  |0.0136|

Correction algorithm ablation:

thresh=0.05                                                                                                     
% |gsm8k|      3|strict-match    |     5|exact_match|0.7066|±  |0.0125|                                                                                                       
% |     |       |flexible-extract|     5|exact_match|0.7058|±  |0.0126|    

thresh=0.2                                                                                                     
% |gsm8k|      3|strict-match    |     5|exact_match|0.7218|±  |0.0123|                                                                                                       
% |     |       |flexible-extract|     5|exact_match|0.7240|±  |0.0123|  

thresh=0.3

% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.7301|±  |0.0122|
% |     |       |flexible-extract|     5|exact_match|0.7324|±  |0.0122|

kernel size ablation:
GSM8k
8, 16, 32

8:                                    
% |gsm8k|      3|strict-match    |     5|exact_match|0.7316|±  |0.0122|                                                                                                       
% |     |       |flexible-extract|     5|exact_match|0.7339|±  |0.0122|  

24:

% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.7195|±  |0.0124|
% |     |       |flexible-extract|     5|exact_match|0.7255|±  |0.0123|

32:
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.6929|±  |0.0127|
% |     |       |flexible-extract|     5|exact_match|0.6998|±  |0.0126|

sparsity ablation:
0.4 0.3 0.2 


cats++
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=True,kernel_size=16,spr=0.4,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.7104|±  |0.0125|
% |     |       |flexible-extract|     5|exact_match|0.7111|±  |0.0125|
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=True,kernel_size=16,spr=0.3,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.6315|±  |0.0133|
% |     |       |flexible-extract|     5|exact_match|0.6558|±  |0.0131|


cats
% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=False,kernel_size=16,spr=0.4,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.3131|±  |0.0128|
% |     |       |flexible-extract|     5|exact_match|0.3184|±  |0.0128|

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=False,kernel_size=16,spr=0.3,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.0121|±  |0.0030|
% |     |       |flexible-extract|     5|exact_match|0.0303|±  |0.0047|

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,cats=True,check=False,kernel_size=16,spr=0.2,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.0030|±  |0.0015|
% |     |       |flexible-extract|     5|exact_match|0.0167|±  |0.0035|

griffin++:

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=True,kernel_size=16,spr=0.4,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.6657|±  | 0.013|
% |     |       |flexible-extract|     5|exact_match|0.6672|±  | 0.013|


% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=True,kernel_size=16,spr=0.3,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.6217|±  |0.0134|
% |     |       |flexible-extract|     5|exact_match|0.6300|±  |0.0133|

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=True,kernel_size=16,spr=0.2,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.5102|±  |0.0138|
% |     |       |flexible-extract|     5|exact_match|0.5716|±  |0.0136|

griffin:

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=False,kernel_size=16,spr=0.4,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.2206|±  |0.0114|
% |     |       |flexible-extract|     5|exact_match|0.2244|±  |0.0115|

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=False,kernel_size=16,spr=0.3,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.0660|±  |0.0068|
% |     |       |flexible-extract|     5|exact_match|0.0697|±  |0.0070|

% xhf (pretrained=meta-llama/Meta-Llama-3-8B-Instruct,griffin=True,check=False,kernel_size=16,spr=0.2,thr=0.1), gen_kwargs: (None), limit: None, num_fewshot: None, batch_size: 1
% |Tasks|Version|     Filter     |n-shot|  Metric   |Value |   |Stderr|
% |-----|------:|----------------|-----:|-----------|-----:|---|-----:|
% |gsm8k|      3|strict-match    |     5|exact_match|0.0099|±  |0.0027|
% |     |       |flexible-extract|     5|exact_match|0.0281|±  |0.0045|

Can put into appendices:

some tasks will do well with sparse. We can preserve its advantage:

CoQA (sparsity 0.4, 0.3, 0.2)

cats ++
0.587 0.6032 0.5923

cats
0.5850 0.6018 0.586 

griffin ++
0.6155 0.6165 0.6212

griffin
0.6155 0.6165 0.6212

along with truthfulQA / $lf\_eval$ results

% \begin{table*}
%     \caption{}
%     \label{tab:L40}
%     \centering
%     \resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{l|c|c|c|c}
%         \toprule
%          & \multirow{2}{*}{{\bf GSM8K}} & \multirow{2}{*}{{\bf CoQA}} & \multirow{2}{*}{{\bf AGIEval (Math)}} & \multirow{2}{*}{{\bf MMLU}} \\
%           & &  & &  \\
%         \midrule
%  Llama2-7B-chat & 0.2396/0.2426 & 0.5982/0.7580 &0.072& 0.4925 \\
% Llama2-7B-chat-FSparse & 0.1979/0.2017& 0.5898/0.7540 & 0.077 &0.4768 \\
% Llama2-7B-chat-FSparse-\Sys & 0.2282/0.2312  & 0.5908/0.7540  & 0.081& 0.4670 \\
% Llama2-7B-chat-CSparse  & 0.1334/0.1380& 0.6117/0.7639 &0.065 & 0.4637\\
% Llama2-7B-chat-CSparse-\Sys  & 0.2183/0.2206 & 0.6117/0.7664&  0.078& 0.4794 \\
%         \midrule
%  Llama2-8B-chat & 0.7551/0.7544 & 0.6153/0.7825 &0.213 & 0.6231\\
%  Llama2-8B-chat-FSparse & 0.5868/0.5891& 0.5828/0.7577& 0.172& 0.5304\\
% Llama2-8B-chat-FSparse-\Sys  &0.7263/0.7271  &0.5868/0.7591  & 0.196 &0.5709 \\
% Llama2-8B-chat-CSparse  & 0.3859/0.3874& 0.6003/0.7735& 0.154& 0.5558\\
% Llama2-8B-chat-CSparse-\Sys  &0.6679/0.6702  &  0.6005/0.7728&  0.178 & 0.6003\\
%         \midrule
%  Llama2-13B-chat & 0.3563/0.3662 & 0.6408/0.7896 & 0.092 & 0.5317 \\
%   Llama2-13B-chat-FSparse & 0.3222/0.3275 &0.6320/0.7837 &0.087 & 0.5082\\
% Llama2-13B-chat-FSparse-\Sys  & 0.3533/0.3571& 0.6340/0.7859 &0.089 & 0.5219\\
% Llama2-13B-chat-CSparse  & 0.2714/0.2767& 0.6350/0.7841&0.088 & 0.5127\\
% Llama2-13B-chat-CSparse-\Sys  & 0.3412/0.3487 & 0.6363/0.7847& 0.1& 0.5127 \\
%         \midrule
%  Llama2-7B &0.1319/0.1365 & 0.6388/0.7735 & 0.101 & 0.4520 \\
%   Llama2-7B-FSparse & 0.1107/0.1145&  0.6352/0.7697&  0.09& 0.4435\\
% Llama2-7B-FSparse-\Sys  & 0.1183/0.1198 & 0.6352/0.7697 & 0.092& 0.4415\\
% Llama2-7B-CSparse  & 0.0796/0.0864&0.6338/0.7700 & 0.086& 0.4213\\
% Llama2-7B-CSparse-\Sys  & 0.1152/0.1168& 0.6372/0.7709 &0.093 & 0.4317\\
%         \midrule
%  Llama2-8B & 0.4973/0.5042 & 0.6727/0.8055 & 0.163 & 0.5754 \\
%   Llama2-8B-FSparse & 0.3154/0.3192& 0.6625/0.7984 & 0.152& 0.5349\\
% Llama2-8B-FSparse-\Sys  &0.4306/0.4352 &0.6625/0.7984 &0.154 &0.5532  \\
% Llama2-8B-CSparse  & 0.1986/0.2062& 0.6633/0.7977 &0.131 & 0.5049\\
% Llama2-8B-CSparse-\Sys  &0.4193/0.4261 & 0.6670/0.7995& 0.15& 0.5428\\
%         \bottomrule
%     \end{tabular}}
% \end{table*}





% \begin{table*}
%     \caption{}
%     \label{tab:L40}
%     \centering
%     \resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{l|c|c|c|c|c|c}
%         \toprule
%          & \multirow{2}{*}{{\bf GSM8K}} & \multirow{2}{*}{{\bf CoQA}} & \multirow{2}{*}{{\bf TruthfulQA}} & \multirow{2}{*}{{\bf MMLU}} & \multirow{2}{*}{{\bf IfEval}}& \multirow{2}{*}{{\bf HumanEval}}\\
%           & &  & &  & \\
%         \midrule
%  Llama2-7B-chat & 0.2396/0.2426 & 0.5982/0.7580 & 0.4492/0.3843 & 0.4925 & 0.2902/0.4137 \\
% Llama2-7B-chat-FSparse & 0.1979/0.2017& 0.5898/0.7540 & 0.4406/0.3684 &0.4768 &0.3124/0.4281\\
% Llama2-7B-chat-FSparse-\Sys & 0.2282/0.2312 (15) & 0.5908/0.7540 (16) & 0.4382/0.3733 (14)& 0.4670 (14)&0.3124/0.4305(13.5)\\
% Llama2-7B-chat-CSparse  & 0.1334/0.1380& 0.6117/0.7639 &0.4247/0.3831 & 0.4637&0.2699/0.4257\\
% Llama2-7B-chat-CSparse-\Sys  & 0.2183/0.2206 (12.6)& 0.6117/0.7664 (14)& 0.4406/0.3941 (9) & 0.4794 (10) &0.2976/0.4257(5.5)\\
%         \midrule
%  Llama2-8B-chat & 0.7551/0.7544 & 0.6153/0.7825 & 0.4823/0.3623 & 0.6231 & 0.3919/0.5300 \\
%  Llama2-8B-chat-FSparse & 0.5868/0.5891& 0.5828/0.7577& 0.5288/0.3476 & 0.5304&0.3808/0.5192\\
% Llama2-8B-chat-FSparse-\Sys  &0.7263/0.7271 (14) &0.5868/0.7591 (15) & 0.5177/0.3501 (13)&0.5709 (13) &0.4011/0.5408 (13.5)\\
% Llama2-8B-chat-CSparse  & 0.3859/0.3874& 0.6003/0.7735& 0.4639/0.3268& 0.5558&0.3494/0.4892\\
% Llama2-8B-chat-CSparse-\Sys  &0.6679/0.6702 (13) & 0.6005/0.7730 (12) & 0.4859/0.3525 (9) & 0.6003(10)&\\
%         \midrule
%  Llama-2-13B-Chat & 0.3563/0.3662 & 0.6408/0.7896 & 0.4272/0.3525 & 0.5317 & 0.3142/0.4293 \\
%   Llama-2-13B-Chat-FSparse & 0.3222/0.3275 &0.6320/0.7837 & 0.4162/0.3476& 0.5082&0.2717/0.3933\\
% Llama-2-13B-Chat-FSparse-\Sys  & 0.3533/0.3571& 0.6320/0.7837 & 0.4162/0.3537& 0.5219 (14)&0.2919/0.4133(13)\\
% Llama-2-13B-Chat-CSparse  & 0.2714/0.2767& 0.6350/0.7841&0.3782/0.3231 & 0.5127&0.2902/0.4185\\
% Llama-2-13B-Chat-CSparse-\Sys  & 0.3412/0.3487 & 0.6363/0.7847&0.3758/0.3244 & 0.5127 (10)&0.2791/0.4173(5.5)\\
%         \midrule
%  Llama2-7B &0.1319/0.1365 & 0.6388/0.7735 & 0.3207/0.3048 & 0.4520 & 0.1848/0.3189 \\
%   Llama2-7B-FSparse & 0.1107/0.1145&  0.6352/0.7697& 0.3550/0.3366 & 0.4435&0.1774/0.3094\\
% Llama2-7B-FSparse-\Sys  & 0.1183/0.1198 & 0.6352/0.7697 & 0.3488/0.3305& 0.4415(15) &0.1830/0.3141(15.5)\\
% Llama2-7B-CSparse  & 0.0796/0.0864&0.6338/0.7700 & 0.3035/0.2827& 0.4213&0.1959/0.3213\\
% Llama2-7B-CSparse-\Sys  & 0.1152/0.1168& 0.6352/0.770 & 0.2913/0.2778& 0.4317 (13)&0.1830/0.3153(14)\\
%         \midrule
%  Llama2-8B & 0.4973/0.5042 & 0.6727/0.8055 & 0.4198/0.3696 & 0.5754 & 0.1109/0.2062 \\
%   Llama2-8B-FSparse & 0.3154/0.3192& 0.6625/0.7984 & 0.4945/0.4443& 0.5349&0.1072/0.2050\\
% Llama2-8B-FSparse-\Sys  &0.4306/0.4352 &0.6625/0.7984 &0.4835/0.4345 &0.5532 (14) &0.0961/0.1942(15.5)\\
% Llama2-8B-CSparse  & 0.1986/0.2062& 0.6633/0.7977 &0.4492/0.4064 & 0.5049&0.1017/0.1954\\
% Llama2-8B-CSparse-\Sys  &0.4193/0.4261 & &0.4553/0.4113 & 0.5428(12)&0.1091/0.2062(14)\\
%         \bottomrule
%     \end{tabular}}
% \end{table*}
